EOGS++: Earth Observation Gaussian Splatting with Internal Camera Refinement and Direct Panchromatic Rendering

Recently, 3D Gaussian Splatting has been introduced as a compelling alternative to NeRF for Earth observation, offering competitive reconstruction quality with significantly reduced training times. In this work, we extend the Earth Observation Gaussian Splatting (EOGS) framework to propose EOGS++, a novel method tailored for satellite imagery that directly operates on raw high-resolution panchromatic data without requiring external preprocessing. Furthermore, leveraging optical flow techniques we embed bundle adjustment directly within the training process, avoiding reliance on external optimization tools while improving camera pose estimation. We also introduce several improvements to the original implementation, including early stopping and TSDF post-processing, all contributing to sharper reconstructions and better geometric accuracy. Experiments on the IARPA 2016 and DFC2019 datasets demonstrate that EOGS++ achieves state-of-the-art performance in terms of reconstruction quality and efficiency, outperforming the original EOGS method and other NeRF-based methods while maintaining the computational advantages of Gaussian Splatting. Our model demonstrates an improvement from 1.33 to 1.19 mean MAE errors on buildings compared to the original EOGS models

==> chapter/table_results.tex <==
\begin{table*}[ht]
        \centering
        \begin{tabular}{lllllllllllllll}
        & \rot{Panchromatic} & \rot{Optical-Flow} & \rot{Reset+Early Stopping} & \rot{TSDF}   & \rot{JAX 004} & \rot{JAX 068} & \rot{JAX 214} & \rot{JAX 260} & \rot{JAX Mean $\downarrow$}  & \rot{IARPA 001} & \rot{IARPA 002} & \rot{IARPA 003} & \rot{IARPA Mean $\downarrow$} & \rot{Time}\\ \midrule
        EOGS      & \xmark & \xmark & \xmark & \xmark & 0.89 & 1.01 & 1.63 & 1.24 & 1.19 & 1.38 & 1.70 & 1.03 & 1.37 & 0.05\\
        EO-NeRF   & \xmark & \xmark & \xmark & \xmark & 1.02 & 1.03 & 1.55 & 1.24 & 1.21 & 1.32 & 1.63 & 1.18 & 1.38 & 15   \\
        SAT-NGP   & \xmark & \xmark & \xmark & \xmark & 1.03 & 1.26 & 2.17 & 1.43 & 1.47 & 1.34 & 1.85 & 1.62 & 1.60 & 0.42 \\
        EOGS++    & \cmark & \cmark & \cmark & \cmark & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & H.hh\\ \midrule
        Ablations & \cmark & \xmark & \xmark & \xmark & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & H.hh\\
                  & \xmark & \cmark & \xmark & \xmark & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & H.hh\\
                  & \xmark & \xmark & \cmark & \xmark & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & H.hh\\
                  & \xmark & \xmark & \xmark & \cmark & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & H.hh\\ \bottomrule
        \end{tabular}
        \caption{\TODO{BHO}}
        
    \end{table*}
\begin{table*}[]
\begin{tabular}{llllllllllllllll}
 &
  \rot{Panchromatic} &
  \rot{Optical-Flow} &
  \rot{Reset+Early Stopping} &
  \rot{TSDF} &
  \rot{ Bundle-Adjusted-RPC} &
  \rot{JAX 004} &
  \rot{JAX 068} &
  \rot{JAX 214} &
  \rot{JAX 260} &
  \rot{JAX Mean $\downarrow$} &
  \rot{IARPA 001} &
  \rot{IARPA 002} &
  \rot{IARPA 003} &
  \rot{IARPA Mean $\downarrow$} &
  \rot{Time }\\ \cline{1-5} \cline{7-16} 
EOGS                  & \xmark     & \xmark & \xmark & \xmark & \cmark & 0.89 & 1.01 & 1.63 & 1.24 & 1.19 & 1.38 & 1.70 & 1.03 & 1.37 & 0.05 \\
EO-NeRF               & \xmark     & \xmark & \xmark & \xmark & \cmark & 1.02 & 1.03 & 1.55 & 1.24 & 1.21 & 1.32 & 1.63 & 1.18 & 1.38 & 15   \\
SAT-NGP               & \xmark     & \xmark & \xmark & \xmark & \cmark & 1.03 & 1.26 & 2.17 & 1.43 & 1.47 & 1.34 & 1.85 & 1.62 & 1.60 & 0.42 \\
EOGS++ ( bd)          & \cmark     & \xmark & \cmark & \cmark & \cmark & 1.82 & 1.05 & 1.84 & 1.86 &  1.64    & \textbf{1.22} & 1.81 & 1.09 & 1.37 & 0.3  \\
EOGS++ (OF)           & \cmark     & \cmark & \cmark & \cmark & \xmark & 6.6  & 1.52 & 2.67 & 6.0  & 4.2 & 1.34 & 1.85 & 1.23 & 1.47 & 0.5  \\ \hline
Ablations (raw RPC)   & \cmark     & \xmark & \xmark & \xmark & \xmark & 7.74 & 3.95 & 4.39 & 4.45 & 5.13 & 2.11 & 2.4  & 2.44 & 2.32 & 2    \\
Optical flow          & \cmark (?) & \cmark & \xmark & \xmark & \xmark & ?    & 1.34 & 3.64 & 2.3  &  & 1.36 & 1.95 & 1.53 &  1.61     & 0.5  \\
Reset+ early stopping & \cmark     & \cmark & \cmark & \xmark & \xmark & 6.6  & 1.52 & 2.67 & 6.0  & 4.2 & 1.34 & 1.85 & 1.23 & 1.47 & H.hh \\
TSDF                  & \xmark     & \xmark & \xmark & \cmark & \xmark & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & X.XX & H.hh \\ \hline
\end{tabular}
\caption{Mean absolute errors on the elevation, in meters, and the corresponding training time for various baseline, when ignoring the foliage areas.  }
\label{tab:exp_main_v2}
\end{table*}




  \begin{table*}[ht]
  \centering
  \begin{tabular}{rccccccllc}
   &
    \multicolumn{2}{c}{IARPA 001} &
    \multicolumn{2}{c}{IARPA 002} &
    \multicolumn{2}{c}{IARPA 003} &
    \multicolumn{2}{l}{Mean IARPA} &
    time (hours) \\ \cline{2-9}
                                   & no FM & FM   & no FM & FM   & no FM & FM   & no FM & FM   &    \\ \hline
  EO-Nerf$\sim$\cite{eonerf}       &       &      &       &      &       &      &       &      &    \\ \hline
  raw RPC                          & 2.34  & 2.20 & 2.93  & 2.73 & 2.17  & 2.07 & 2.48  & 2.33 & 15 \\
  RPC internal BA. &
    1.50 &
    1.41 &
    \textbf{1.88} &
    \textbf{1.66} &
    1.42 &
    1.35 &
    1.60 &
    \textbf{1.47} &
    15 \\
  RPC bundle adjusted &
    \textbf{1.42} &
    1.27 &
    \textbf{1.79} &
    \textbf{1.56} &
    1.31 &
    1.24 &
    \textbf{1.51} &
    \textbf{1.36} &
    15 \\ \hline
  \namemodel                       &       &      &       &      &       &      &       &      &    \\ \hline
  raw RPC (OnlyPAN)                & 2.33  & 2.11 & 2.7   & 2.4  & 2.58  & 2.44 & 2.54  & 2.32 & 2  \\
  learn Worldview Matrix (onlyPAN) & 1.87  & 1.56 & 2.38  & 2.0  & 2.61  & 2.41 & 2.29  & 1.99 & 2  \\
  flowmatching (onlyPAN) &
    \textbf{1.50} &
    \textbf{1.34} &
    2.05 &
    1.85 &
    \textbf{1.41} &
    \textbf{1.23} &
    1.65 &
    \textbf{1.47} &
    0.5 \\
  RPC bundle adjusted (onlyPAN) &
    1.43 &
    \textbf{1.22} &
    2.0 &
    1.81 &
    \textbf{1.24} &
    \textbf{1.09} &
    1.56 &
    1.37 &
    0.3 \\ \hline
  \end{tabular}
  \caption{ Mean absolute error on the elevation [meters] and the corresponding training time for \nameeonerf and different bundle adjustment algorithm, when considering
  the whole area (no mask) or when ignoring foliage areas (FM).}
  \label{tab:exp_main}
  \end{table*}
